Adaptive Quotient Filters

Adaptive filters, such as telescoping and adaptive cuckoo filters, update their representation upon detecting a false positive to avoid repeating the same error in the future. Adaptive filters require an auxiliary structure, typically much larger than the main filter and often residing on slow storage, to facilitate adaptation. However, existing adaptive filters are not practical and have seen no adoption in real-world systems due to two main reasons. Firstly, they offer weak adaptivity guarantees, meaning that fixing a new false positive can cause a previously fixed false positive to come back. Secondly, the sub-optimal design of the auxiliary structure results in adaptivity overheads so substantial that they can actually diminish the overall system performance compared to a traditional filter. In this paper, we design and implement AdaptiveQF, the first practical adaptive filter with minimal adaptivity overhead and strong adaptivity guarantees, which means that the performance and false-positive guarantees continue to hold even for adversarial workloads. The AdaptiveQF is based on the state-of-the-art quotient filter design and preserves all the critical features of the quotient filter such as cache efficiency and mergeability. Furthermore, we employ a new auxiliary structure design which results in considerably low adaptivity overhead and makes the AdaptiveQF practical in real systems.

==> Makefile <==
ALL = main.pdf
TEXFILES = main abstract defines evaluation includes conclusion implementation intro related title plots acknowledgments throughput_plots workload_plots blacklist-filter disk_throughput_plots
FIGURES =
LATEXMKOPTS = -pdf -dvi- -pdflatex="pdflatex --shell-escape %O %S"
LATEX = pdflatex --shell-escape
BIBFILES = bibliography 
#BIBFILES = bibliography BFJ-bigdata-papers allpapers

########### Shouldn't require configuration below here ##########

# run "make CONT=1" for continuous compilation
ifdef CONT
	LATEXMKOPTS += -pvc
	FORCED = .PHONY
endif

all: $(ALL)

$(ALL): $(TEXFILES:=.tex) $(FIGURES) $(BIBFILES:=.bib)

# How to compile a .tex file to a .pdf file
%.pdf: %.tex $(FORCED)
	@if (command -v latexmk > /dev/null) ; then latexmk $(LATEXMKOPTS) $< ; \
	else $(LATEX) $<; bibtex $@; $(LATEX) $<; $(LATEX) $<; fi 

#
# Rules for converting various figure formats to pdf
#

%.pdf_tex: %.svg
	inkscape -A $(@:.pdf_tex=.pdf) --export-latex $<

%.pdf: %.svg
	inkscape -A $@ $<

%.pdf: %.dia
	dia --nosplash -e $(@:.pdf=.eps) $(@:.pdf=.dia) 
	epstopdf $(@:.pdf=.eps)

%.pdf: %.fig
	fig2dev -L pdftex $< $@

%.pdf_t: %.fig %.pdf
	fig2dev -L pdftex_t -p $(@:.pdf_t=.pdf) $< $@

%.pstex_t: %.fig
	fig2dev -L pstex_t -p $(@:.pstex_t=.pstex) $< $@
	fig2dev -L pstex $< $(@:.pstex_t=.pstex)

.PHONY:

clean:
	latexmk -C


==> copyright.tex <==
\copyrightyear{2021}
\acmYear{2021}
\setcopyright{rightsretained}
\acmConference[SIGMOD '21]{Proceedings of the 2021 International Conference on Management of Data}{June 20--25, 2021}{Virtual Event, China}
\acmBooktitle{Proceedings of the 2021 International Conference on Management of Data (SIGMOD '21), June 20--25, 2021, Virtual Event, China}\acmDOI{10.1145/3448016.3452841}
\acmISBN{978-1-4503-8343-1/21/06}


==> lower-bound.tex <==
% Backup of the full proof of the lower bound

\subsection{Lower bound for static \YesNo List filters}

In \cite{Reviriego2021BlacklistFilter} they sketch a space lower bound for the static \yesno list problem. But the claim is unclear and the math is extremely sloppy. Here is a better version of that.

\begin{theorem}
Suppose $u \geq 10 (n^2/\epsilon + m^2)$ (for some value of $10$). Further, suppose $\epsilon \leq 1/2$. Then, the number of bits used by a static \yesno list filter is at least
\[
\min\limits_{\epsilon' \in (0, \epsilon]} n \lg(1/\epsilon') + \epsilon' m \lg e + \Omega(1).
\]
\end{theorem}
Before proving the theorem, we note that an analysis of the function $f(\epsilon') = n \lg(1/\epsilon') + \epsilon' m \lg e + \Omega(1)$ with $\epsilon' \in (0, \epsilon]$ reveals that:
\begin{itemize}
	\item if $\epsilon \leq n/m$, then $f$ attains its minimum at $\epsilon' = \epsilon$;
	\item if $\epsilon > n/m$, then $f$ attains its minimum at $\epsilon' = n/m$. 
\end{itemize}
Hence, the lower bound can be equivalently stated as
\[
\left\{
\begin{array}{cc}
n \lg(1/\epsilon) + \epsilon m \lg e + \Omega(1) & \text{if $\epsilon \leq n/m$}\\
n \lg(m/n) + n \lg e + \Omega(1) & \text{otherwise}
\end{array}
\right..
\]

\begin{proof}
Let $D$ be a \yesno list filter that uses at most $\ell$ bits on all inputs $(S, T, \epsilon)$ with $|S| = n$ and $|T| = m$. For any random bit string $r$, denote $D_r(S, T, \epsilon)$ the instance of $D$ with randomness $r$ on input $(S, T, \epsilon)$. We will use the following standard information-theoretic argument: If $R$ is an upper bound on the number of inputs that each instance of $D$ can represent, and $I$ is the number of inputs,  then there are at least $I/R$ different instances, which means that $2^\ell \geq I/R$, or $\ell \geq \lg(I/R)$.

Unfortunately, this only yields a good lower bound if $R$ is small, but there's nothing preventing some instances to represent a large number of inputs. The key idea is that we can always find a subset of instances that represent all inputs, but such that, individually, each of those instances can only represent few inputs. Then we can use the information-theoretic argument on this subset of instances.

Fix a particular input $(S_1, T_1, \epsilon)$. For any string of random bits $r$, let $\calI_r := D_r(S_1, T_1, \epsilon)$ be the resulting instance. For every $x \in U \setminus (S_1 \cup T_1)$, we have $\Pr\limits_r[\text{$\calI_r$ answers \yes on $x$}] \leq \epsilon$. By linearity of expectation,
\[
\E\limits_r[|\{x \in U \setminus(S_1 \cup T_1) : \text{$\calI_r$ answers \yes on $x$}\}|] \leq \epsilon.
\]
Therefore, there exists an $r$ such that $\calI_r$ answers \yes on some fraction $\epsilon' \leq \epsilon$ of elements in $U \setminus (S_1 \cup T_1)$. We call an instance that errs on at most a fraction $\epsilon$ of elements \defn{good}. The previous argument shows that for every input there is a good instance that represents it. In particular, the collection of good instances represent all inputs.

The number of inputs that $\calI_r$ can represent is at most
\begin{align*}
R(\epsilon') &:= {n + \epsilon'(u - n - m) \choose n}{u - (n + \epsilon'(u - n - m)) \choose m}\\
&\leq \frac{(n + \epsilon'(u - n - m))^n (m + (1-\epsilon')(u - n - m))^m}{n! m!}.
\end{align*}
(Notice that it's not necessarily true that $\calI_r$ can represent at most $R(\epsilon)$ inputs, because $R(\epsilon')$ is not monotonically increasing on $\epsilon'$.)
Therefore, an upper bound of the number of inputs every good instance can represent is
\[
R := \sup\limits_{\epsilon' \in (0, \epsilon]} R(\epsilon').
\]
On the other hand, the number of inputs is
\[
I = {u \choose n}{u-n \choose m} \geq \frac{\Omega((u - n - m)^{n + m})}{n! m!}.
\]
Thus,
\begin{align*}
\ell &\geq \lg(I/R)\\
&= \lg\left(\frac{I}{\sup\limits_{\epsilon' \in (0, \epsilon]} R(\epsilon')}\right)\\
&= \inf\limits_{\epsilon' \in (0, \epsilon]} \lg(I / R(\epsilon'))\\
&\geq \inf\limits_{\epsilon' \in (0, \epsilon]} \lg\left(\frac{\Omega((u - n - m)^{n+m})}{(n + \epsilon'(u-n-m))^n(m + (1-\epsilon')(u-n-m))^m}\right).
\end{align*}
Let's bound the second term in the denominator. Since $u \geq \Omega(m^2) \cap \Omega(n)$ and $\epsilon'$ is bounded away from $1$, then
\[
m \leq \frac{1}{m}(1-\epsilon')(u-n-m),
\]
and, thus,
\[
(m + (1-\epsilon')(u-n-m))^m \leq (1 + 1/m)^m (1-\epsilon')^m(u-n-m)^m \leq O((1-\epsilon')^m(u-n-m)^m).
\]
Plugging this into the lower bound yields
\[
\ell \geq \inf\limits_{\epsilon' \in (0, \epsilon]} \lg\left(\frac{\Omega((u - n - m)^{n})}{(n + \epsilon'(u-n-m))^n(1-\epsilon')^m}\right).
\]

Now we'll split the infimum into two cases, namely $\epsilon' < n^2 / (u-n-m)$ or not. Let $\ell_{1}$ and $\ell_{2}$ be the infimums when $\epsilon' < n^2 / (u-n-m)$ and otherwise, respectively; then, $\ell \geq \min\{\ell_1, \ell_2\}$. We do this in order to bound the first term in the denominator. Intuitively, when $\epsilon'(u-n-m) < n^2$, then $\epsilon'$ is extremely small, and thus the filter is essentially a dictionary. In this case, the lower bound $\ell_1$ will be very large. In the other case, when $\epsilon'$ is not extremely small, will get a much smaller and more accurate lower bound $\ell_2$. Since we're taking the minimum over the two cases, only $\ell_2$ survives.

Suppose $\epsilon'(u-n-m) < n^2$. Then,
\[
(n + \epsilon'(u-n-m))^n < (n + n^2))^n \leq O(n^{2n}).
\]
Then,
\[
\ell_1 \geq \lg\left(\frac{\Omega((u-n-m)^n)}{O(n^{2n})}\right) \geq \lg\left(\frac{\Omega(u^n)}{O(n^{2n})}\right) = \Omega(n \log(u/n^2)),
\] 
where the second inequality is because $u = \Omega(n^2) \cap \Omega(m^2)$.

On the other hand, if $\epsilon'(u-n-m) \geq n^2$, we have
\[
(n + \epsilon'(u - n - m))^n = O(\epsilon'^n(u-n-m)^n),
\]
so
\begin{align*}
\ell_2 &\geq \inf\limits_{\epsilon'  \in [n^2/(u-n-m), \epsilon]} \lg\left(\frac{\Omega(1)}{\epsilon'^n (1-\epsilon')^m}\right)\\
&= \inf\limits_{\epsilon'  \in [n^2/(u-n-m), \epsilon]} (n \lg(1/\epsilon') + m \lg(1/(1-\epsilon'))) + \Omega(1)\\
&\geq \inf\limits_{\epsilon'  \in [n^2/(u-n-m), \epsilon]} (n \lg(1/\epsilon') + \epsilon' m \lg e) + \Omega(1) \tag{as $\ln(1/(1-x)) \geq x$ for all $x \in (0, 1)$}\\
&\geq \inf\limits_{\epsilon'  \in (0, \epsilon]} (n \lg(1/\epsilon') + \epsilon' m \lg e) + \Omega(1)
\end{align*}
Thus,
\[
\ell_2 \geq
\left\lbrace
\begin{array}{ll}
	n \lg(1/\epsilon) + \epsilon m \lg e + \Omega(1) & \text{if $\epsilon \leq n/m$}\\
	n \lg(m/n) + n \lg e + \Omega(1) & \text{otherwise}
\end{array}
\right..
\]
Finally, since $u = \Omega(n^2/\epsilon)$, both of these cases are smaller than $\Omega(n \log(u / n^2)) \leq \ell_1$, so the theorem follows.
\end{proof}


==> related.tex <==
% !TEX root =  main.tex

\section{Related Work}\label{sec:related}

\subsection{Filters}

For decades, the Bloom filter~\cite{Bloom70} was essentially the only game in town, but
Bloom filters are suboptimal in terms of space usage, running time, and data locality, and they support a bare-bones set of operations (insert and lookup).

\depricate{
In particular,
Bloom filters consume $\log(e)\, \opt$ space, which is roughly $\log(e)\approx
1.44$ times more than the lower bound of $\opt + \Omega(n)$
bits~\cite{CarterFG78}.
%In contrast, for a set $S$ taken from a universe $U$, where $|U|=u$, an
%  error-free dictionary requires $\Omega(\log {u\choose n}) \approx \Omega(n
%\log u)$ bits.
Bloom filters also incur $\errbits$ cache-line misses on inserts and positive queries, giving them poor insertion and query performance.
}


The Bloom filter has inspired numerous variants~\cite{QiaoLiCh14, PutzeSaSi07,
LuDeDu11, CanimMiBh10, DebnathSeLi11, AlmeidaBaPr07, FanCaAl00, BonomiMiPa06}.
The counting Bloom filter (CBF)~\cite{FanCaAl00} replaces each bit in the Bloom
filter with a $c$-bit saturating counter.  This enables the CBF to support
deletes, but increases the space by a factor of $c$. 
%
The blocked Bloom
filter~\cite{PutzeSaSi07} provides better cache locality than the standard Bloom
filter but does not support deletion.

%The scalable Bloom
%filter~\cite{AlmeidaBaPr07} uses multiple Bloom filters to maintain
%the target false-positive rate $\epsilon$ even when $n$ is unknown. 

The quotient filter (QF)~\cite{PaghPR05,DillingerMa09,BenderFaJo12a,EinzigerFr16} uses a new,
non-Bloom-filter design. It is built on the idea of storing small
fingerprints via Robin Hood hashing~\cite{CelisLaMu85}. It supports insertion, deletion, lookups, resizing, and
merging. The counting quotient filter (CQF)~\cite{PandeyBJP17}, improves upon
the performance of the quotient filter and adds variable-sized counters to count items using
asymptotically optimal space, even in large and skewed datasets.

%This is achieved by using slots originally
%reserved to store the remainders to store count information instead.  The
%metadata bits maintained by the CQF allows this dynamic reuse of remainder slots
%for large counters while still ensuring the correctness of all CQF operations.

%The quotient filter hashes items to a $p$-bit fingerprint and uses
%the upper bits of the fingerprint to select a slot in a table, where it stores
%the lower bits of the fingerprint.  It resolves collisions using a variant of
%linear probing that maintains three metadata bits per slot.  

%The variable-sized counters in the CQF enable the data structure to handle
%highly skewed datasets efficiently. By reusing the allocated space, the CQF
%avoids wasting extra space on counters and naturally and dynamically adapts to
%the frequency distribution of the input data.  The CQF never takes more space
%than a quotient filter for storing the same multiset. For highly skewed
%distributions, like those observed in HTS-based datasets, it occupies only a
%small fraction of the space that would be required by a comparable (in terms of
%false-positive rate) quotient filter.

The cuckoo filter~\cite{FanAnKa14} uses the idea from quotient filters of hashing small
fingerprints but uses cuckoo hashing instead of Robin Hood hashing. The Morton filter~\cite{BreslowJ18} is a variant of the cuckoo filter that is
designed to speed up insertion using optimizations designed for hierarchical
systems.

\subsection{Filters for Blocklists/Requirelists} Chazellete et. al. introduced the Bloomier filter~\cite{chazelle2004bloomier} which was designed to not only guarantee a small false-positive probability but to ensure that a \defn{requirelist}, a pre-specified list of negative elements, would never be false positives. 

Li et. al., present the Seesaw Counting Filter~\cite{seesaw2022} (SSCF), which implements a blocklist/requirelist filter specifically for the URL blocklist problem. The SSCF has an extension for adding requirelist items dynamically, but in order to prevent from introducing false negatives into the filter, it must wait to modify the requirelist until associated buckets have been completely vacated. As a result, adaptations are neither immediate nor guaranteed, and the possibility for dynamic adaptation of the requirelist can only exist in situations with enough volatility to ensure that any given bucket will be completely emptied after a reasonable amount of time. Because our experiments were conducted with large load factors, the SSCF could not be reliably expected to adapt. Moreover, the requirelist becomes less effective as it fills up more of the filter, so the filter would need some way to decide which false positives to adapt to and which to ignore, and it would eventually need to stop making adaptations altogether. As a result, the adaptivity of the SSCF does not apply to the same circumstances as the AQF, so it is excluded from the evaluation.

Reviriego et. al.~\cite{reviriego2021} present the Integrated Filter which also implements a requirelist. All focus on the case where the requirelist is static and known ahead of time. 

\subsection{Adaptive filters}

Adaptive filters are advanced filters that can update their internal representation when informed of a false positive. Adaptive filters also need a way to map the fingerprints stored in the filter to original keys to safely adapt to avoid future false positive keys. Adaptive filters are typically used as a small in-RAM summary the contents of a set in external storage. When the system issues a query $x$ to the external set, if the filter says $x$ is not in the external set the system can skip the unnecessary I/O to access the external set. A false positive means the system will perform an I/O to access the external set and subsequently discover the false positive item is not present.

Mitzenmacher et. al.~\cite{MitzenmacherPR20} proposed the adaptive cucko filter (ACF)~\cite{MitzenmacherPR20}, an adaptive filter based on the cuckoo filter. It is specifically designed to reduce false-positive rate on skew query distributions. Kopelowitz et. al.~\cite{kopelowitz2021support} propose an improved version of the ACF and also show that any strongly adaptive filter must use variable-length fingerprints. As a result all existing variants of the ACF are not strongly adaptive. While the ACF is not strongly adaptive, they show that it is \defn{support optimal}: it guarantees a false-positive rate of at most $\epsilon$ for any \emph{fixed} query sequence.

Bender et. al.~\cite{BenderFaGo18} introduce the broom filter and the notion of strong adaptivity described in this paper. The broom filter is a quotient filter that adapts by extending the fingerprints of elements that cause false positives. Lee et. al.~\cite{lee2021telescoping} introduce the telescoping filter, which is also built using the quotient filter~\cite{PandeyBJP17}. The telescoping filter is strongly adaptive but avoids directly extending fingerprints. They change the remainder (or the tag) stored in the filter by using a different lower-order $r$-bits. Additionally, they maintain a table to record which $r$-bits they have used as a remainder in the filter for the adapted items. As the filter adapts, the size of this table grows (so in this sense their fingerprints are variable-length and strong adaptivity is possible).
 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:



